Good-for-MDPs Automata for Probabilistic Analysis and Reinforcement Learning

We characterize the class of nondeterministic ${\omega}$-automata that can be used for the analysis of finite Markov decision processes (MDPs). We call these automata `good-for-MDPs' (GFM). We show that GFM automata are closed under classic simulation as well as under more powerful simulation relations that leverage properties of optimal control strategies for MDPs. This closure enables us to exploit state-space reduction techniques, such as those based on direct and delayed simulation, that guarantee simulation equivalence. We demonstrate the promise of GFM automata by defining a new class of automata with favorable properties - they are B\"uchi automata with low branching degree obtained through a simple construction - and show that going beyond limit-deterministic automata may significantly benefit reinforcement learning.

==> chocolates.tex <==
\begin{figure}
  \centering
  \begin{tikzpicture}[
    every text node part/.style={align=center},
    every state/.style={fill=safecellcolor}]
    \begin{scope}
      \node[state,initial above] (S0) at (0,0) {$q_0$};
      \node[state] (S1) [below=1.75 cm of S0] {$q_1$};
      \path[->]
      (S0) edge [loop right] node [right=1mm] {$*$} ()
      edge node [label={right:$*$}] {} (S1)
      (S1) edge [loop right] node [accepting dot,label={right:$p_1$}] {} ();
      \foreach \x [evaluate=\x as \prev using int(\x-1)] in {2,...,5} {
        \node[state] (S\x) [below=1.75 cm of S\prev] {$q_\x$};
        \path[->]
        (S\prev) edge node [label={right:$\bar{p}_\prev$}] {} (S\x)
        (S\x) edge [loop right] node [accepting dot,label={right:$p_\x$}] {} ();
      }
      \node[state] (T) [below=1.75 cm of S5] {$q_t$};
      \path[->]
      (S5) edge node [label={right:$\bar{p}_5$}] {} (T)
      (T) edge [loop right] node [right=1mm] {$*$} ();
    \end{scope}
    \begin{scope}[xshift=7.5cm,yshift=-1cm]
      \node[state] (S1) {$q_1$};
      \path[->]
      (S1) edge [loop above] node [accepting dot, label={$p_1$}] {} ();
      \foreach \x [evaluate=\x as \prev using int(\x-1)] in {2,...,5} {
        \node[state] (S\x) [below=2.2 cm of S\prev] {$q_\x$};
        \path[->]
        (S\x) edge [loop above] node [accepting dot, label={$p_\x$}] {} ();
      }
      \node[state,initial] (S0) [left=4cm of S3]
      {$q_0$};
      \node[state] (T) [right=4cm of S3] {$q_t$};
      \path[->]
      (S0) edge [loop above] node[above=1mm] {$*$} ()
      (T) edge [loop right] node[right=1mm] {$*$} ();
      \foreach \x in {1,...,5} {
        \path[->]
        (S0) edge node [sloped,above=1mm,pos=0.55] {$p_\x$} (S\x)
        (S\x) edge node [sloped,above=1mm,pos=0.45] {$\bar{p}_\x$} (T);
      }
    \end{scope}
  \end{tikzpicture}
  \caption{Serial (left) and parallel (right) automata for $\bigvee_i
    \eventually\always p_i$.  A transition
    labeled $*$ is enabled for all letters of the alphabet; a
    transition labeled $\bar{p}_i$ is enabled for all letters for
    which $p_i$ is false.}
  \label{fig:choco1}
\end{figure}

\begin{figure}
  \begin{tikzpicture}[
    every text node part/.style={align=center},
    every state/.style={fill=safecellcolor}]
    \begin{scope}
      \node[state,initial] (Q0) at (0,0) {$q_0$};
      \node[state] (Q1) [right=1.75 cm of Q0] {$q_1$};
      \path[->]
      (Q0) edge [loop above] node [accepting dot,label={$y$}] {} ()
      edge [loop below] node [label={below:$\neg y$}] {} ()
      edge node [accepting dot,label={$x$}] {} (Q1)
      (Q1) edge [loop above] node [accepting dot,label={$x$}] {} ();
    \end{scope}
    \begin{scope}[xshift=4.5cm,yshift=-3cm]
      \node[state,initial] (Q0) at (0,0) {$0|$};
      \node[state,inner sep=1pt] (Q1) [above right=2.5cm and 4.5cm of Q0] {$0,1|1$};
      \node[state,inner sep=1pt] (Q2) [below=5 cm of Q1] {$0,1|$};
      \node[state] (Q3) [right=3 cm of Q1] {$1|$};
      %\node[state] (Q4) [below=2 cm of Q3] {$\emptyset$};
      \path[->]
      (Q0) edge [loop above] node [accepting dot,label={$\neg x \wedge
        y$}] {} ()
      edge [loop below] node {$\neg x \wedge \neg y$} ()
      edge node [inner sep=1pt] {$x \wedge \neg y$} (Q1)
      edge node [accepting dot,label={$x \wedge y$}] {} (Q2)
      (Q1) edge [loop above] node {$x \wedge \neg y$} ()
      edge node [accepting dot,label={$x \wedge \neg y$}] {} (Q3)
      edge [bend left=25,inner sep=1pt] node {$\neg x \wedge \neg y$} (Q0)
      edge [bend right] node [accepting dot,label={$\neg x \wedge y$}]
      {} (Q0)
      edge [bend left=50] node [accepting dot,label={right:$x \wedge y$}]
      {} (Q2)
      (Q2) edge [loop below] node [accepting dot,label={below:$x
        \wedge y$}] {} ()
      edge [bend left=10,swap] node {$x \wedge \neg y$} (Q1)
      edge [bend right=25,inner sep=1pt,swap] node {$\neg x \wedge \neg y$} (Q0)
      edge [bend left] node [accepting dot,label={$\neg x \wedge y$}]
      {} (Q0)
      (Q3) edge [loop above] node [accepting dot,label={$x$}] {} ()
      %edge node {$\neg x$} (Q4)
      %(Q4) edge [loop below] node {$\top$} ()
      ;
    \end{scope}
    \begin{scope}[yshift=-4cm]
      \node[state,initial] (Q0) at (0,0) {$q_0$};
      \node[state] (Q1) [right=2 cm of Q0] {$q_1$};
      \node[state] (Q2) [below=1.75 cm of Q1] {$q_2$};
      \path[->]
      (Q0) edge [loop above] node [accepting dot,label={$y$}] {} ()
      edge [loop below] node [label={below:$\neg y$}] {} ()
      edge [bend left] node [accepting dot,label={$x \wedge \neg y$}] {} (Q1)
      (Q1) edge [loop above] node [accepting dot,label={$x \wedge \neg
        y$}] {} ()
      edge [bend left] node [accepting dot, label={$y$}] {} (Q0)
      edge node {$\neg x \wedge \neg y$} (Q2)
      (Q2) edge [loop below] node {$\neg y$} ()
      edge node [accepting dot, label={below:$y$}] {} (Q0);
    \end{scope}
  \end{tikzpicture}
  \caption{Three GFM automata for
    $(\eventually\always x) \vee (\always\eventually y)$.  Eager (top
    left), ``wait and see'' (right), and forgiving (bottom left).  The
    ``wait and see'' automaton is the result of the construction of
    Theorem~\ref{theo:slim} applied to the eager automaton.}
  \label{fig:forgiveness-2}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% TeX-PDF-mode: t
%%% End:


==> slimFigureOld.tex <==
\begin{comment}
\begin{figure}
  \centering
  \begin{tikzpicture}
    \node[state,initial above,fill=safecellcolor] (S0) at (0,0) {$0$};
    \node[state,fill=safecellcolor] (S1) [right=2.25cm of S0] {$1$};
    \path[->]
    (S0) edge[bend left] node {$a,b$} (S1)
         edge[loop left] node {$a,b$} ()
    (S1) edge[bend left] node[accepting dot, label={$a$}] {} (S0)
    ;
  \end{tikzpicture}

  \begin{tikzpicture}[every text node part/.style={align=center}]
    \node[state,darkgreen,fill=goodcellcolor] (S0) at (4,3)
    {$\{0\}$};
    \coordinate [left=1cm of S0] (ild);
    \node[state,darkgreen,fill=goodcellcolor] (S01) [right=2.75cm of
    S0] {$\{0,1\}$};
    \node[state,fill=badcellcolor] (S1-e) [below left=2.5cm and 1.25cm of
    S0] {$\{1\}$\\$\emptyset$};
    \node[state,initial below,fill=safecellcolor] (S0-e) [right=2.75cm
    of S1-e] {$\{0\}$\\$\emptyset$};
    \node[state,fill=safecellcolor] (S01-e) [right=2.75cm of S0-e]
    {$\{0,1\}$\\$\emptyset$}; 
    \node[state,fill=safecellcolor] (S01-0) [right=2.75cm of S01-e]
    {$\{0,1\}$\\$\{0\}$}; 
    \path[->]
    (ild) edge[darkgreen] (S0)
    (S0) edge[darkgreen] node {$a,b$} (S01)
         edge[darkgreen,swap] node[sloped,above,pos=0.3] {$a,b$} (S1-e)
         edge[darkgreen] node[sloped,pos=0.3,above] {$a,b$} (S0-e)
         edge[darkgreen] node[sloped,pos=0.2,above] {$a,b$} (S01-e)
    (S01) edge[darkgreen,loop right] node {$a,b$} ()
         edge[darkgreen,swap] node[pos=0.7,sloped,above] {$a,b$} (S1-e)
         edge[darkgreen] node[pos=0.7,sloped,above] {$a,b$} (S0-e)
         edge[darkgreen] node[sloped,above,pos=0.6] {$a,b$} (S01-e)
    (S1-e) edge node[accepting dot, label={$a$}] {} (S0-e)
    (S0-e) edge node {$a,b$} (S01-e)
    (S01-e) edge[bend left] node {$a$} (S01-0)
    edge [loop above, looseness=4, out=120, in=60] node {$b$} (S01-e)
    (S01-0) edge[out=200, in=-20] node[accepting dot, label={$a,b$}] {} (S01-e)
    (S01-0) edge[red,dashed,out=240,in=-60] node[accepting
    dot,label={$a,b$}] {} (S01-e);
  \end{tikzpicture}
  \caption{An NBW, a suitable LDBA, and a slim automaton for
    $\always\eventually a$}
  \label{fig:slim-GFa-backup}
\end{figure}
\end{comment}

\begin{figure}[t]
  \centering
  \begin{tikzpicture}[every text node part/.style={align=center}]
    \begin{scope}
      \node[state,darkgreen,fill=goodcellcolor,inner sep=1pt] (S01) at (4,3) {$\{0,1\}$};
      \coordinate [left=1cm of S01] (ild);
      \node[state,fill=badcellcolor,inner sep=1pt] (S1-e) [below left=2.5cm and 2.75cm of
      S01] {$\{1\}$\\$\emptyset$};
      \node[state,fill=badcellcolor,inner sep=1pt] (S0-e) [right=2.75cm
      of S1-e] {$\{0\}$\\$\emptyset$};
      \node[state,initial below,fill=safecellcolor,inner sep=1pt] (S01-e) [right=2.75cm of S0-e]
      {$\{0,1\}$\\$\emptyset$}; 
      \node[state,fill=safecellcolor,inner sep=1pt] (S01-0) [right=2.75cm of S01-e]
      {$\{0,1\}$\\$\{0\}$}; 
      \path[->]
      (ild) edge[darkgreen] (S01)
      (S01) edge[darkgreen,loop right] node {$a,b$} ()
      edge[darkgreen,swap] node[sloped,above] {$a,b$} (S1-e)
      edge[darkgreen] node[sloped,above] {$a,b$} (S0-e)
      edge[darkgreen] node[sloped,above] {$a,b$} (S01-e)
      (S1-e) edge node[accepting dot, label={$a$}] {} (S0-e)
      (S0-e) edge node {$a,b$} (S01-e)
      (S01-e) edge[bend left=45] node {$a$} (S01-0)
      edge [loop above, looseness=4, out=120, in=60] node {$b$} (S01-e)
      (S01-0) edge node[accepting dot, label={$a,b$}] {} (S01-e)
      (S01-0) edge[red,dashed,out=225,in=-45] node[accepting
      dot,label={$a,b$}] {} (S01-e);
    \end{scope}
    \begin{scope}[xshift=10cm,yshift=2.75cm]
      \node[state,initial above,fill=safecellcolor] (S0) at (0,0) {$0$};
      \node[state,initial above,fill=safecellcolor] (S1) [right=2.25cm of S0] {$1$};
      \path[->]
      (S0) edge[bend left] node {$a,b$} (S1)
      edge[loop left] node {$a,b$} ()
      (S1) edge[bend left] node[accepting dot, label={$a$}] {} (S0)
      ;
    \end{scope}
  \end{tikzpicture}
  \caption{An NBA for $\always\eventually a$ (in the upper right
    corner) together with an SLDBA and a slim NBA constructed
    from it.  The SLDBA and the slim NBA are shown sharing their common
    part.  State $\{0,1\}$, produced by the subset construction, is
    the initial state of the SLDBA, while state
    $(\{0,1\},\emptyset)$---the initial state of the breakpoint
    construction---is the initial state of the slim NBA.  States
    $(\{1\},\emptyset)$ and $(\{0\},\emptyset)$ are states of the
    breakpoint construction that only belong to the SLDBA because they
    are not reachable from $(\{0,1\},\emptyset)$.  The transitions out
    of $\{0,1\}$, except the self loop, belong to $\Delta_{SB}$.  The
    dashed-line transition from $(\{0,1\},\{0\})$ belongs to
    $\gamma_{2,1}$}
  \label{fig:slim-GFa}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% TeX-PDF-mode: t
%%% End:


==> slimGFM.tex <==
\subsection{Are Slim Automata Good for Reinforcement Learning?}
\label{sec:slim-is-good}

The low branching degree of slim automata suggests that they may be
suited to reinforcement learning of $\omega$-regular objectives.  To
test this hypothesis we have run the Mungojerrie tool of Hahn \emph{et
  al.}\ \cite{Hahn19} on all the MDPs in the result table of
\cite{Hahn19}, whose properties are not recognized by deterministic
B\"uchi automata.  We omit all the models with deterministic automata
because those are both slim and limit deterministic; therefore they
cannot be used to study the differences between the two types of
automata.  We added a new property for model \texttt{deferredFG} and a
large MDP, which we designed, to the examples from \cite{Hahn19}.  For
all models and properties we consider, we are interested in comparing
learning speed when using slim automata, and when using limit
deterministic automata.  To that effect, we find the number of
episodes at which good strategies are found most of the times, unless
this number exceeds $10^7$.  The hyperparameters were optimized for
each experiment.

We use {Mungojerrie} \cite{Hahn19} for MDP model checking and model-free
reinforcement learning.  MDPs are coded in the Prism language
\cite{kwiatk11}, while automata are written in the standard HOA format
\cite{Babiak15}.  In all experiments we used Q-learning to compute
optimal strategies.  All the limit deterministic automata were
handcrafted for minimum size.  All the slim automata were produced by
translating the LTL specifications to nondeterministic B\"uchi
automata with SPOT \cite{Duret-LutzLFMRX16}, and then applying the
construction of Section~\ref{ssec:slim}, which we implemented in ePMC
\cite{HahnLSTZ14}.

\begin{table}[t]
  \caption{Learning results.  The 
    hyperparameters are: $\zeta$, $1$ minus the probability of reward
    on an accepting transition, $\epsilon$, exploration rate,
    $\alpha$, learning rate, tol, minimum value for $Q$ values to be
    deemed different, ep-l, episode length, and ep-n, number of
    episodes.  Times are in seconds.}
  \label{tab:experiments}
  \centering
  %\small
  \begin{tabular}[c]{l|ccccccccccccc}
    Name & type & aut. & product & $p$ & time & $\zeta$ & $\varepsilon$ & $\alpha$ & tol & ep-l & ep-n \\\hline
    \multirow{2}{*}{\texttt{twoPairs}}     & \textsc{sldba} & 4   & 25      & 1    & 0.05  &  \multirow{2}{*}{0.99} &  \multirow{2}{*}{0.1}  &  \multirow{2}{*}{0.2}  &  \multirow{2}{*}{0}   &  \multirow{2}{*}{30} & 3500 \\
                          & Slim  & 13  & 36      & 1    & 0.09  &       &       &       &      &     & 5000 \\
    \multirow{2}{*}{\texttt{trafficNtk}}  & \textsc{sldba} & 13  & 1680    & 1    & 0.02  &  \multirow{2}{*}{0.95} &  \multirow{2}{*}{0.25} &  \multirow{2}{*}{0.2}  &  \multirow{2}{*}{0}   &  30 &  200 \\
                          & Slim  & 22  & 3415    & 1    & 0.13  &       &       &       &      & 400 & 3500 \\
    \multirow{2}{*}{\texttt{knuthYao}}     & \textsc{sldba} & 3   & 53      & 1    & 0.01  &  \multirow{2}{*}{0.99} &  \multirow{2}{*}{0.2}  &  \multirow{2}{*}{0.2}  &  \multirow{2}{*}{0}   & \multirow{2}{*}{100} & 1000 \\
                          & Slim  & 5   & 46      & 1    & 0.01  &       &       &       &      &      &   50 \\
    \multirow{2}{*}{\texttt{strat1}}       & \textsc{sldba} & 4   & 15      & 1    & 0.01  &  \multirow{2}{*}{0.95} &  \multirow{2}{*}{0.01} &  \multirow{2}{*}{0.2}  &  \multirow{2}{*}{0}   &  \multirow{2}{*}{30} &   15 \\
                          & Slim  & 9   & 19      & 1    & 0.01  &       &       &       &      &     &   20 \\
    \multirow{2}{*}{\texttt{deferredFG}}   & \textsc{sldba} & 3   & 122     & 0    & 135.9 & \multirow{2}{*}{0.999} &   \multirow{2}{*}{0.1} &  \multirow{2}{*}{0.1}  &  \multirow{2}{*}{0}   &  \multirow{2}{*}{50} & $10^7$ \\
                          & Slim  & 5   & 64      & 1    & 0.43  &       &       &       &      &     & 700  \\
    \multirow{2}{*}{\texttt{chocolates}}   & \textsc{sldba} & 7   & 1087668 & 0    & 84.0  & \multirow{2}{*}{0.9}   & \multirow{2}{*}{0.01}  & \multirow{2}{*}{0.3}   &  \multirow{2}{*}{0}   &20000& $10^7$ \\
                          & Slim  & 275 & 1034706 & 1    & 6.9   &       &       &       &      & 200 & 1200
    \end{tabular}
    \vspace*{-4mm}
\end{table}

The results of our experiments are summarized in
Table~\ref{tab:experiments}.  The leftmost column lists the models.
Example \texttt{twoPairs} is used in \cite{Hahn19} to show that an
optimal strategy that uses only one Rabin pair may not exist when the
property requires more than one pair.  Example \texttt{trafficNtk} is
the traffic network example from \cite{Sadigh14}.  Example
\texttt{knuthYao} is a model of repeated rolls of Knuth and Yao's fair
die, where the learning agent learns to continue until a six is
rolled.  Example \texttt{strat1} is a small MDP, for which the transition
probabilities make rewards infrequent.  Example \texttt{deferredFG} is
a difficult example for reinforcement learning because short-term
rewards lead to suboptimal strategies; the property to be satisfied is
$\eventually \always p$.  Example \texttt{chocolates} presents the
learner with the task to stop eating chocolates from a set of
boxes exactly when the last chocolate is about to be eaten.

The column labeled ``type'' identifies the type of automaton.  The
column labeled ``aut.'' reports the number of states of the
automaton.  The column labeled ``product'' reports the number of
states in the product of the automaton and MDP used for model
checking.  (Note, however, that model-free learning does not build the product.)  The
column labeled ``$p$'' gives the probability of satisfaction of each
property with the strategy computed by learning.  (All properties are
satisfied with probability $1$ under optimal strategies.)  The column
labeled ``time'' reports the CPU time required by Q learning (the
median of three runs).  The remaining columns give the values of
learning parameters.  When a parameter has the same value for both
types of automata, it is specified only once.

While results are preliminary and based on a small data set, they show
a promising trend: The fact that slim automata tend to be larger than
optimized SLDBAs seems to be compensated by the better guidance that
they provide for learning when to make the nondeterministic ``jumps.''

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% TeX-PDF-mode: t
%%% End:

